ReMasker: Imputing Tabular Data with Masked Autoencoding

We present ReMasker, a new method of imputing missing values in tabular data by extending the masked autoencoding framework. Compared with prior work, ReMasker is both simple -- besides the missing values (i.e., naturally masked), we randomly ``re-mask'' another set of values, optimize the autoencoder by reconstructing this re-masked set, and apply the trained model to predict the missing values; and effective -- with extensive evaluation on benchmark datasets, we show that ReMasker performs on par with or outperforms state-of-the-art methods in terms of both imputation fidelity and utility under various missingness settings, while its performance advantage often increases with the ratio of missing data. We further explore theoretical justification for its effectiveness, showing that ReMasker tends to learn missingness-invariant representations of tabular data. Our findings indicate that masked modeling represents a promising direction for further research on tabular data imputation. The code is publicly available.

==> analysis.tex <==
\section{Analysis}



==> background.tex <==
\section{Preliminaries}


==> method.tex <==
\section{\system}

Next, we present the design of \system and detail the implementation of its key components. At a high level, \system is a transformer-based generative model to synthesize tabular data. We invent {\em random projection transformer}, a new design of the transformer block to tackle the challenge of arbitrary inter-attribute dependencies; we use mode-specific encoding to handle the heterogeneity of different attributes; and we develop a suite of strategies to stabilize the training of \system.


\subsection{Random-Projection Transformer}

\missingfigure{RP-Transformer}




\subsection{Training Recipe}


==> notuse.tex <==


% \section{Introduction}

% Here, we present an alternative use of the transformer in the task of tabular data synthesis. 
% We present \system\footnote{\system: \underline{Ta}bular \underline{T}ransformer-based  \underline{G}enerative \underline{A}dversarial \underline{N}etwork.}, a transformer-based generative model for tabular data, which integrate two transformers in a generative adversarial network (GAN) framework,
% one as the generator and the other as the discriminator. However, although the transformer architecture has been successfully applied in the tasks of generating text~\citep{transformer} and images~\citep{transgan,styleswin}, implementing \system for synthesizing tabular data represents non-trivial challenges. First, while image or text data often shows coherency across different parts (e.g., spatial coherence in the structure and color of images), tabular data can have arbitrarily complex dependencies between different attributes. Further, unlike text and image data which is relatively homogeneous, tabular data often demonstrates vast heterogeneity among different types of attributes (e.g., numerical versus categorical). Finally, the training of GANs is notoriously unstable, often resulting in mode collapse~\citep{mode-collapse}. 

% To address the aforementioned challenges, this paper presents a suite of designs and strategies towards realizing \system. Specifically, 

% \begin{itemize}
    
%     \item Architecture -- Rather than directly stacking multiple regular transformer blocks, which is unable to capture arbitrary dependencies and scales poorly with the number of attributes (i.e., quadratic complexity), we propose RP-Transformer, a new design of the transformer block, random-partitioning Transformer (RP-Transformer). RP-Transformer divides different attributes into random partitions and only computes self-attention within each partition. Further, to introduce cross-partition connections while maintaining the computation efficiency, we introduce alternative partitioning schemes in consecutive RP-Transformer blocks. 
    
%     \item Encoding -- We adopt different encoding schemes for numerical and categorical attributes. For categorical attributes, we use one-hot encoding, while for numerical attributes, we use mode-specific encoding~\citep{ctgan}, which estimates the modes of each attribute and adaptively generates the encodings.
    
%     \item Training -- we explore a number of strategies to improve the training stability, including positioning encoding, layer normalization, and data augmentation. We further conduct extensive ablation studies to characterize the effectiveness of different ingredients.
% \end{itemize}


% \section{Related Work}

% Here, we survey relevant literature in three categories. 

% {\bf  Generative adversarial network --} As a general framework of generative model, GANs have gained surging popularity in a range of tasks~\citep{Goodfellow:2014:nips}. Yet, the training of GANs is notoriously unstable. A variety of strategies have been proposed including the Wasserstein loss~\citep{wgan}, progressive training~\citep{progressive-training}, and spectral normalization~\citep{spectral-norm}.

% {\bf  Tabular data synthesis --} Due to its wide range of applications, tabular data synthesis has attracted intensive research. The first line of work treats each attribute as a random variable, models a joint distribution over different attributes, and then samples from this distribution~\citep{vine-copula}. Yet, the modeling capabilities of these methods is limited by the types of underlying distributions. Another line of work uses deep generative models such as VAEs and GANs~\citep{medgan,tablegan,ctgan} to generate tabular data, especially healthcare records. \ting{todo}

% {\bf  Transformer-based data synthesis --} Originally proposed for NLP tasks, the transformer has emerged as a dominating architecture design~\citep{transformer}, in which multi-head self-attention and MLP layers are stacked to capture both short- and long-term correlation between words. Recent work has explored the use of transformers in the computer vision domain by treating each image as a sequence of visual words~\citep{vit}. A set of recent work have integrated the transformer modules into image generation models~\citep{transgan,styleswin,gat}, which achieve performance comparable to CNN-based generative models.

% Yet, to our best knowledge, none of existing work has attempted to apply the transformer architecture in the task of tabular data synthesis.


% \section{\system}

% Next, we present the design of \system and detail the implementation of its key components. At a high level, \system is a transformer-based generative model to synthesize tabular data. We invent {\em random projection transformer}, a new design of the transformer block to tackle the challenge of arbitrary inter-attribute dependencies; we use mode-specific encoding to handle the heterogeneity of different attributes; and we develop a suite of strategies to stabilize the training of \system.


% \section{Evaluation}

% {\bf Setting --} We conduct an empirical evaluation of \system on the SDGym\footnote{SDGym: \url{https://github.com/sdv-dev/SDGym}} benchmark.


% {\bf Data Fidelity --} We evaluate the fidelity of the synthesized data by comparing it with the original data.




% {\bf Data Utility --} We further evaluate the utility of the synthesized data by different models in downstream tasks. 


% \begin{table}[!hp]
%     \centering
%     \renewcommand{\arraystretch}{1.15}
%     \begin{tabular}{ccccc}
% & \multicolumn{2}{c}{GM Simulated} & \multicolumn{2}{c}{BN Simulated} \\
% Method & syn & test & syn & test  \\
% \hline  
% \hline
% Identity & -2.61 & -2.61 & -9.33 & -9.36  \\
% \hline
% TableGAN & -8.24 & -4.12 & -11.84 & -10.47 \\
% CTGAN &  -5.72 & -3.40 & -11.67 & -10.60 \\
% TVAE & {\bf -2.65} & -5.42 & -6.76 & {\bf -9.59}\\
% \hline
% TaTGAN & -2.81 & {\bf -3.30} & {\bf -6.70} & -9.70 \\
%     \end{tabular}
%     \caption{Benchmark results over three sets of experiments, Gaussian mixture simulated data, Bayesian network simulated data, and real data.}
%     \label{tab:my_label}
% \end{table}



% {\bf Ablation Study --} We conduct an ablation study to explore the impact of different components of \system on data fidelity and utility.

